Generative Adversarial Loops

AI research progress can be viewed as the interaction between two processes: benchmark creation and method discovery. Historically, both were driven by human intelligence. However, recent advances in AI have accelerated automated method discovery, while automated benchmark creation has received comparatively less attention. To enable self-advancing systems, we propose Generative Adversarial Loop (GAL), a generator-discriminator framework alternating between two agentic searches: (1) a discriminator that generates adversarial data to expose weaknesses in current systems, and (2) a generator that discovers algorithms to overcome them. We apply this framework to approximation algorithms for efficient inference. Unlike existing auto research systems, which primarily focus on algorithm discovery, GAL introduces a discriminator agent that automates goalpost setting by continually searching for weaknesses in the current algorithm. We demonstrate adversarial data generation across four tasks: KV compression, sparse video generation, sparse attention, and context extension, where the discriminator identifies weaknesses in state of the art techniques. We further show that GAL enables autonomous improvement, with newly discovered algorithms improving not only on adversarially generated data, but also on established benchmarks. Specifically, GAL improves CompactorPress on KV compression with Qwen3-4B at 4x, raising performance on the discriminator dataset from 0.35 to 0.97, while also outperforming RULER-HARD (+0.77 pts). For context extension, GAL boosts Dual Chunk Attention from 0.20 to 0.90 on the discriminator dataset, while yielding gains on standard benchmarks(ScienceFiction (+6 pts) and PG19 32K (-0.33 PPL)). GAL thus provides a path toward autonomous goalpost setting and algorithmic improvement, where AI systems continually discover their own weaknesses and develop methods to overcome them.

==> sections/abstract.tex <==
Benchmarks have become a primary driver of progress in modern AI, enabling standardized evaluation and rapid iteration across increasingly capable systems. While they accelerate advancement, they can also encourage directional optimization, where models improve disproportionately on benchmark-specific distributions rather than developing broadly robust capabilities. Nevertheless, analyzing failures on difficult evaluations remains one of the most effective ways to identify weaknesses and guide improvement. Traditionally, humans have discovered these weaknesses and constructed harder benchmarks, effectively moving the goalpost as AI systems improve. As models become more capable, however, identifying their limitations is itself becoming challenging. At the same time, auto-research frameworks are accelerating algorithmic and model improvement, making human-driven benchmark creation an increasingly significant bottleneck. This motivates automated discovery of weaknesses in AI systems and, consequently, automated benchmark creation. We propose Generative Adversarial Loops, a generator-discriminator framework for autonomous improvement that alternates between two agentic searches: (1) Discriminator: adversarial data generation to expose weaknesses in current systems, and (2) Generator: algorithmic discovery to overcome them. We apply this framework to approximation algorithms for efficient inference. Unlike existing auto-research systems, which primarily focus on algorithm discovery, our approach adds a discriminator agent that automates goalpost setting by continually searching for weaknesses in the current algorithm. We demonstrate adversarial data generation across four tasks: KV compression with FastKVZip, sparse video generation with SVG, sparse attention with TopK, and context extension with DCA. In each case, the discriminator identifies weaknesses in state-of-the-art algorithms. In a case study on DCA, a few generative adversarial loops produce improved algorithms that not only perform well on adversarially generated data but also improve performance on established benchmarks. Generative Adversarial Loops thus provide a path toward autonomous goalpost setting and algorithmic improvement, where AI systems continually discover their own weaknesses and develop methods to overcome them.


==> sections/abstract_1.tex <==
\looseness=-1 Research progress in machine learning can be understood as the interaction between two complementary processes: benchmark creation and method discovery. Benchmark creation is a discriminative process that generates data highlighting weaknesses in existing systems and sets new goalposts, while method discovery is the scientific process of devising methods that overcome these weaknesses and improve performance on the benchmark. Traditionally, human intelligence drove progress on both fronts. However, the increasing contribution of AI to scientific discovery has accelerated one process, while the other remains largely human-driven, creating a bottleneck to further progress. To realize self-advancing systems, we propose Generative Adversarial Loops, a generator-discriminator framework for autonomous improvement that alternates between two agentic searches: (1) Discriminator: adversarial data generation to expose weaknesses in current systems, and (2) Generator: algorithmic discovery to overcome them. We apply this framework to approximation algorithms for efficient inference. Unlike existing auto-research systems, which primarily focus on algorithm discovery, our approach adds a discriminator agent that automates goalpost setting by continually searching for weaknesses in the current algorithm. We demonstrate adversarial data generation across four tasks: KV compression with FastKVZip, sparse video generation with SVG, sparse attention with TopK, and context extension with DCA. In each case, the discriminator identifies weaknesses in state-of-the-art algorithms. In two tasks: context extension with DCA and KV compression with Compactor press, we demonstrate that a few generative adversarial loops improve algorithms over adversarially generated data. In some cases, the improved algorithms also improve performance on established benchmarks. Generative Adversarial Loops thus provide a path toward autonomous goalpost setting and algorithmic improvement, where AI systems continually discover their own weaknesses and develop methods to overcome them.

\begin{comment}
In a case study on DCA, a few generative adversarial loops produce improved algorithms that not only perform well on adversarially generated data but also improve performance on established benchmarks. Generative Adversarial Loops thus provide a path toward autonomous goalpost setting and algorithmic improvement, where AI systems continually discover their own weaknesses and develop methods to overcome them.
\end{comment}


==> sections/abstract_2.tex <==
Research progress in AI can be understood as the interaction between two complementary processes: benchmark creation and method discovery. Historically, both processes were driven by human intelligence. However, recent advances in AI have significantly accelerated automated method discovery, while automated benchmark creation has received comparatively less attention. To realize truly self advancing systems, we propose Generative Adversarial Loop (GAL), a generator discriminator framework that alternates between two agentic searches: (1) a discriminator that generates adversarial data to expose weaknesses in current systems, and (2) a generator that discovers algorithms to overcome them. We apply this framework to approximation algorithms for efficient inference. Unlike existing auto research systems, which primarily focus on algorithm discovery, GAL introduces a discriminator agent that automates goalpost setting by continually searching for weaknesses in the current algorithm. We demonstrate adversarial data generation across four tasks: KV compression, sparse video generation, sparse attention, and context extension, where the discriminator identifies weaknesses in state of the art techniques. We further show that GAL enables autonomous improvement for KV compression and context extension, with newly discovered algorithms improving not only on adversarially generated data, but also, in some cases, on established benchmarks. GAL thus provides a path toward autonomous goalpost setting and algorithmic improvement, where AI systems continually discover their own weaknesses and develop methods to overcome them. Code: https://anonymous.4open.science/r/generative-adversarial-loops


==> sections/box.tex <==
\begin{figure*}[t]
\centering
\begin{tcolorbox}[
  enhanced,
  colback=boxgray,
  colframe=black!55,
  boxrule=0.6pt,
  arc=5pt,
  width=\textwidth,
  left=7pt,
  right=7pt,
  top=6pt,
  bottom=8pt
]
\begin{minipage}[t]{0.31\textwidth}
\textbf{1. Adversary}

\vspace{1.8cm}
\end{minipage}\hfill
\begin{minipage}[t]{0.31\textwidth}
\textbf{2. Validation}

\vspace{1.8cm}
\end{minipage}\hfill
\begin{minipage}[t]{0.31\textwidth}
\textbf{3. $B_0$}

\vspace{1.8cm}
\end{minipage}

\vspace{8pt}

\begin{minipage}[t]{0.31\textwidth}
\textbf{4. $B_1$}

\vspace{1.8cm}
\end{minipage}\hfill
\begin{minipage}[t]{0.31\textwidth}
\textbf{5. Evolution results}

\vspace{1.8cm}
\end{minipage}\hfill
\begin{minipage}[t]{0.31\textwidth}
\textbf{6. Short Explanation}

\vspace{1.8cm}
\end{minipage}
\end{tcolorbox}
\caption{Template for an adversarial-evaluation case study.}
\label{fig:box-template}
\end{figure*}


==> sections/case_studies.tex <==
\input{utility/box1}
In this section, we describe the problem domains we target, the algorithms we use to represent the state of the art in each domain, and representative adversarial examples discovered by the GAL discriminator, along with their interpretation. \apd{Add exact settings , models etc details as captions to the figure boxes.}

\subsection{Sparse Video Generation}    

\textbf{Problem Statement and Efficiency Algorithm.}
State-of-the-art video generation is typically performed using diffusion models. These models iteratively refine a video over multiple diffusion steps, with each step requiring computation over the sequence of tokens representing the video. As video resolution and duration increase, this sequence can become extremely long, making each diffusion step increasingly compute-intensive. Consequently, generating only a few seconds of high-resolution video can require tens of minutes even on high-performance GPUs. An effective approach to reducing this cost is to perform \emph{sparse prefill}, which reduces the attention computation while preserving the quality of the generated video.

One state-of-the-art approach is SVG (Sparse Video Generation)~\cite{xi2025sparse}. SVG observes that video attention exhibits two distinct patterns - \emph{spatial} and \emph{temporal} attention patterns. It identifies which patterns the heads belong to, and applies different sparsity patterns to each type of head. The authors show that SVG can substantially reduce computation while maintaining generation quality close to that of dense video generation. In particular, SVG reports PSNR\footnote{PSNR and SSIM are comparative metrics where higher is better} values of approximately 28--29, SSIM around 0.9, and LPIPS\footnote{LPIPS is a comparative metric where lower is better} around 0.1--0.12, with image quality and temporal consistency comparable to, and in some cases better than, dense generation.

\textbf{Example Adversary and Explanation.}
Running the GAL discriminator, we were able to identify adversarial prompts that cause SVG to deviate substantially from dense video generation. One such example is shown in Figure~\ref{fig:svg-box}. For this prompt, the relative PSNR and SSIM are substantially lower, while LPIPS is higher, indicating a larger deviation from the video produced by the dense model. 

The adversarial prompt requests a high-resolution video involving complex interactions of light, creating a challenging generation setting. Such prompts appear to expose a weakness in the sparsity patterns used by SVG: attention that can be safely omitted for typical video-generation prompts may become important when the scene contains fine-grained spatial structure and complex temporal interactions. Thus, while SVG performs well on standard benchmarks, the adversarial example demonstrates that its approximation can break down under specific, systematically generated inputs.

\subsection{Context Extension}
\textbf{Problem Statement and Efficiency Algorithm.}
Extending the context window of a model is computationally expensive. Even in traditional model development, models are often first trained with shorter context windows and subsequently extended to longer contexts in stages. While training models directly on long contexts is expensive, the demand for longer contexts is rapidly increasing due to emerging applications and the shift toward long-lived agents. This motivates the development of training-free methods that can extend a model's effective context window beyond its native context length.

Dual Chunk Attention (DCA)~\cite{an2024training} is a state-of-the-art method for context extension and is natively supported in vLLM~\cite{kwon2023efficient}, with particularly strong results on the Qwen family of models. DCA addresses the out-of-distribution relative positions encountered when a model processes contexts longer than those seen during training. It does so by remapping token positions based on the relative distance between each key and the query. As illustrated in box figure (see parts (3,4)) for DCA, DCA maps tokens from distant chunks into a shared local positional range from $0$ to $C$, where $C$ is the chunk size, while tokens from nearby chunks are positioned immediately preceding the query. In the literature, DCA has demonstrated strong context extension capabilities, typically achieving $2\times$--$4\times$ extension and, in some cases, extending beyond this range while preserving perplexity and downstream retrieval performance.

\textbf{Example Adversary and Explanation.}
Using the GAL discriminator, we identify adversarial patterns that cause DCA to fail substantially. One such pattern is shown in Figure~\ref{fig:dca-box}. The discriminator generates a program parameterized by the context length. At the native context length, the base model successfully solves the problem. However, when the same problem is extended to $4\times$ the native context window, the DCA-enabled model fails.

The adversarial pattern exploits the interaction between DCA's positional remapping and the location of the retrieval information. Specifically, the relevant retrieval information is placed at the boundary of a chunk. Although DCA preserves relative positioning locally within each chunk, its remapping can cause tokens belonging to the same retrieval pattern to be scattered across different relative positions when the information lies near a chunk boundary. For a distant query, this scattering changes the positional structure of the retrieval information relative to the query. As a result, the model may fail to recognize and retrieve the relevant information, despite the information itself being present in the context.

\begin{figure*}[t]
\noindent
\input{utility/kvpress_box}%
\par\vspace{-1.5pt}%
\input{utility/pqcache_box}%
\end{figure*}

\subsection{KV Compression}

\textbf{Problem Statement and Efficiency Algorithm.}
Long context processing and long form generation with autoregressive models gives rise to a unique memory bottleneck: the KV cache. The KV cache consists of intermediate per token embeddings that the model keeps to reduce the computation required to generate a new token. KV caches grow in size linearly with context length and, historically, have had memory footprints comparable to model sizes at long contexts. This forces practitioners to either offload the KV cache to CPU memory or reduce the batch size during serving, which reduces throughput. If we can reduce the memory footprint of the KV cache, we can improve system performance by avoiding offloading and increasing batch sizes. This problem is referred to as KV Compression.

One of the state of the art approaches to KV Compression is KVZip~\cite{kim2026kvzip} and its lighter version, FastKVZip~\cite{kim2026fast}, where we keep a small subset of keys and values that are computed to be important for recovering the entire context that we are compressing. In the literature, these methods show results that maintain model performance up to $4\times$ compression on common retrieval, contextual QA tasks, etc.

\textbf{Example Adversary and Explanation.}
Using the discriminator component of GAL, we identify adversarial patterns that cause FastKVZip to fail substantially. One such pattern is shown in Figure~\ref{fig:kvpress-box}. As we can see, FastKVZip fails significantly, dropping the accuracy score from 0.93 for the uncompressed model to 0.35 for the compressed model.

The adversarial pattern exploits the errors introduced during compression. It creates a ledger and a stale ledger, both of which contain key value pairs. The ledger is placed in the middle of the context, whereas the stale ledger is placed at the end. Every entry of the stale ledger is explicitly marked as stale, and the query specifically asks for the fresh ledger. When the context is comprised of news or articles which are time sensitive, this can be a practical occurrence where stale information is also present in the context.


\subsection{Sparse Decoding}

\textbf{Problem Statement and Efficiency Algorithm.}
Autoregressive decoding in LLMs is memory bound, primarily due to the need to read the huge KV cache from GPU memory to produce a single token. This causes the token throughput of LLMs to be low. To improve this, many approaches to perform sparse attention have been proposed. Sparse attention reduces the amount of memory movement, thereby improving decode throughput. The critical question in sparse attention is choosing the right tokens.

PQCache~\cite{zhang2025pqcache} is one of the state of the art techniques for sparse attention. It chooses the most relevant tokens based on a product quantized representation of the KV cache, which is significantly smaller than the KV cache itself. It is the best top k algorithm on Skylight's sparse attention leaderboard for Qwen mdoels~\footnote{https://sky-light.eecs.berkeley.edu/}. Thus we choose Qwen3-4B-Instruct-2507 with PQCache 2\% sparsity.

\textbf{Example Adversary and Explanation.}
Using the discriminator component of GAL, we identify adversarial patterns that cause PQCache to fail substantially. One such pattern is shown in Figure~\ref{fig:pqcache-box}. As we can see, PQCache performs significantly worse on this pattern.

The adversarial pattern exploits the fact that the nature of most attention is such that it naturally pays more attention to sink tokens (i.e., at the start of the context) and local tokens (near the query). When important keys are embedded in the middle, the lost in the middle phenomenon is observed. Newer models, such as Qwen, after training for long contexts, have largely solved the lost in the middle problem, but when sparsified, the phenomenon shows up again. At higher sparsities (e.g., 5\% or more), this pattern is not adversarial to PQCache.

\begin{figure*}[t]
\centering
\begin{subfigure}[t]{0.48\textwidth}
\centering
\includegraphics[width=\linewidth]{images/kvpress_cursor+gepa_all_models_cost_vs_avg_best_gap.png}
\caption{FastKVZip}
\label{fig:kvpress-all-models}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.48\textwidth}
\centering
\includegraphics[width=\linewidth]{images/dca_cursor+gepa_all_models_cost_vs_avg_best_gap.png}
\caption{DCA}
\label{fig:dca-all-models}
\end{subfigure}
\caption{GEPA and Cursor agent search trajectories across models: average best gap versus cost for FastKVZip (left) and DCA (right) over 10 runs each.}
\label{fig:model-and-agent-ablation}
\end{figure*}

\galpackfalse
\renewcommand{\galpanelht}{4.35cm}
\renewcommand{\galimght}{3.55cm}
\renewcommand{\galbarht}{1.5cm}

\subsection{Cost of Discriminator required to find \texorpdfstring{$b$}{b}}
Figure~\ref{fig:model-and-agent-ablation} shows the cost (in \$) required to find $b$, data points that are adversarial to the efficiency algorithms, across different state of the art models from the Gemini and GPT families. We use GEPA and Cursor as the evolution harness. First, across all models, the solutions evolve towards a higher gap between the unapproximated and approximated inference. This implies that the discriminator recipe works well across different providers and models with different capabilities. What was surprising to us is that lighter models, such as Gemini Flash Lite, Gemini Flash, GPT Luna, etc., are much more effective at generating adversarial data for these harnesses compared to more capable models such as GPT Sol or Gemini Pro. When compared against the costs involved, this disparity becomes even more apparent: we can obtain adversarial data within a fraction of a dollar using lighter models, whereas larger models struggle under the same instructions. 

\textbf{Cost Certificate.}
We can think of the cost required to break an algorithm as a certificate of robustness. Most algorithms in the domain of efficient LLM inference are approximate, and, in principle, there may exist cases where these algorithms deviate from the unapproximated inference. However, the cost required to find such failures provides an indication of how robust these algorithms are. If it is difficult to break a given algorithm for a given efficiency problem, it implies that the algorithm is valuable, covers a broad range of usual use cases, and is worthy of deployment. We refer to this as a \emph{cost certificate} of the algorithm. In the Figure~\ref{fig:model-and-agent-ablation}, we can see that FastKVZip on KVcompression is relatively harder to break than DCA on Context Extension. We find that PQCache which breaks easily at 2\%sparsity does not break that easily at X\%sparsity. \apd{@nidhi / @surya ... need data -- some different cost certificats for pqcache / oracle topk}.


\subsection{Closing the Loop}
\textbf{ContextExtension with DCA}
We run ADRS style evolution as genertor loop of GAL. In this experiment with use Claude coding agent harness. Since, these algorithms are generally part of a bigger repository, we find it useful to run it in such as setup. We run two iterations of complete GAL to discover better algorithms over DCA. The results are presented in Table~\ref{tab:ladder}. We see that the GAL is actually able to produce algorithms that not only cater to adversarial data but also improve performance over standard benchmarks.  \apd{Explain the details of hwo algorithm was improved over DCA} \apd{add kvpress data here.}

\input{tex_figures/dca_ladder_table1}

\textbf{KVCompression with Compactor Press}
Similar to above setup for DCA, we run two iterations of complete GAL to discover better algorithms over Compactor press. The results are presented in Table~\ref{tab:compactor_ladder}. We see that the GAL is actually able to produce algorithms that improve performance on adversarial data while maintaining standard benchmarks. In iterations 1, the adversarial dataset hid a ledger needle among many lookalike mid-context rows; stock Compactor’s global top-k wiped that region, so generator fixed it with stratified keep, reserving budget across sequence tiles so mid-context rows can’t vanish. In iterations 2, the discriminator proposed a multi-hop chain of sparse route IDs that stratified Compactor still dropped; generator fixed it by blending KeyDiff (keep distinctive keys) with attn-protect and value-norm so hop IDs and semantic content both survive.

\input{tex_figures/compactor_ladder_table1}

\apd{Finally: Fit in pages}
\apd{Check format instructions -- do we need checklist? do we need other statements.}




==> sections/dca_example_1.tex <==
\begin{figure}[t]
    \centering
    \begin{tcolorbox}[enhanced, colback=boxgray, colframe=black!55, boxrule=0.6pt,
        arc=5pt, width=\textwidth, left=7pt, right=7pt, top=6pt, bottom=8pt,
        title={\textbf{Worked example --- a boundary-target adversary for DCA
        ($\lambda=2$)}}]
    \footnotesize
    
    %---------------- (a) generator  |  (b) construction ----------------
    \begin{minipage}[t]{0.60\textwidth}
    \textbf{(a) Adversarial generator.} GEPA evolves this length-blind generator; \textbf{bold} marks mutations from the seed.
    \vspace{2pt}
    
    {\scriptsize
    \begin{algorithmic}[1]
    \Require $M$ rows, rng;\ globals $N,\ \lambda N$, chunk size
    \For{$i = 0 \dots M-1$}
        \State id $\gets$ \texttt{"needle-}$i$\texttt{"};\ \ ans $\gets$ random\_code(rng)
        \State depth $\gets \mathrm{Uniform}(\mathbf{0.48},\mathbf{0.52})$ \Comment{seed: U(0.05,0.95)}
        \State needle $\gets$ \texttt{"[[CRITICAL RECORD]] \dots \{ans\}"} \Comment{seed: plain}
        \State \#distractors $\gets \mathbf{12}$ \Comment{seed: 0}
        \State append row(id, ans, needle, depth, \#distractors)
    \EndFor
    \State \Return rows \Comment{harness plants each into base $N$ \& ext $\lambda N$}
    \end{algorithmic}}
    \end{minipage}\hfill
    \begin{minipage}[t]{0.37\textwidth}
    \textbf{(b) Matched construction.} The same target record and question are used
    at both lengths; \emph{only the surrounding filler changes}. At $\lambda=2$, the
    extended input has two DCA chunks. The evolved depth ${\approx}0.5$ places the
    target at their boundary, and the generator inserts 12 same-format distractors.
    \end{minipage}
    
    \vspace{5pt}\hrule\vspace{6pt}
    
    %---------------- visualization: three bars ----------------
    \textbf{(c) Boundary placement under context extension:}\\[4pt]
    \centering
    \begin{tikzpicture}[every node/.style={font=\scriptsize}]
      \def\bh{0.34}
      % --- Native N (one chunk = N) ---
      \node[anchor=west] at (0,2.05+0.5*\bh) {\textbf{Native $N$} (one chunk)};
      \draw[fill=green!8] (4.6,2.05) rectangle (7.6,2.05+\bh);
      \draw[red,very thick] (5.9,2.05)--(5.9,2.05+\bh);
      \node[anchor=west,green!55!black] at (7.75,2.05+0.5*\bh) {retrieved};
      % --- Extended (2N) seed ---
      \node[anchor=west] at (0,1.15+0.5*\bh) {\textbf{Ext.\ $\lambda N$ --- seed}};
      \draw[fill=blue!7] (4.6,1.15) rectangle (10.6,1.15+\bh);
      \draw[dashed] (7.6,1.05)--(7.6,1.15+\bh+0.12);
      \node[font=\tiny] at (6.1,1.15+\bh+0.24) {chunk 0};
      \node[font=\tiny] at (9.1,1.15+\bh+0.24) {chunk 1};
      \draw[red,very thick] (6.0,1.15)--(6.0,1.15+\bh);
      \node[anchor=west,green!55!black] at (10.75,1.15+0.5*\bh) {accuracy $0.90$};
      % --- Extended (2N) evolved ---
      \node[anchor=west] at (0,0.25+0.5*\bh) {\textbf{Ext.\ $\lambda N$ --- evolved}};
      \draw[fill=blue!7] (4.6,0.25) rectangle (10.6,0.25+\bh);
      \draw[dashed] (7.6,0.15)--(7.6,0.25+\bh+0.12);
      \foreach \x in {5.2,6.1,6.9,8.3,9.2,10.0}
          \draw[gray!70] (\x,0.25)--(\x,0.25+\bh);
      \draw[red,very thick] (7.6,0.25)--(7.6,0.25+\bh);
      \node[red,anchor=north,font=\tiny] at (7.6,0.22) {needle at boundary};
      \node[anchor=west,red] at (10.75,0.25+0.5*\bh) {accuracy $0.50$};
    \end{tikzpicture}
    
    \vspace{5pt}\hrule\vspace{5pt}
    \raggedright
    
    %---------------- (c) result  |  (d) explanation ----------------
    \begin{minipage}[t]{0.34\textwidth}
    \centering
    \textbf{(d) Retrieval accuracy}\\[3pt]
    \begin{tabular}{@{}lccc@{}}
    \toprule
     & $N$ & $\lambda N$ & gap \\
    \midrule
    seed    & $1.00$ & $0.90$ & $0.10$ \\
    evolved & $0.95$ & $0.50$ & $\mathbf{0.45}$ \\
    \bottomrule
    \end{tabular}
    \end{minipage}\hfill
    \begin{minipage}[t]{0.63\textwidth}
    \textbf{(e) Why it is difficult.} The generator is length-blind, so the native
    and extended instances differ only in filler. The evolved instance combines
    boundary placement with same-format distractors. DCA's position remapping can
    separate tokens of the boundary-spanning target in the query's effective positional
    view, whereas a distractor can remain locally coherent. This makes the distractors
    more competitive at extended length, while native single-chunk retrieval remains
    reliable. Consequently, the native--extended gap rises from $0.10$ to $0.45$.
    \end{minipage}
    
    \end{tcolorbox}
    \vspace{-3pt}
    \caption{A length-blind adversarial generator for Dual Chunk Attention
    ($\lambda=2$). Relative to the seed, GEPA moves the target to the boundary between
    two extended-context chunks and introduces 12 same-format distractors. The
    resulting instance preserves high native-window accuracy ($0.95$) but reduces
    extended-context accuracy from $0.90$ to $0.50$.}
    \label{fig:dca-example}
    \end{figure}

==> sections/experiments.tex <==
\section{Case Studies}
\label{sec:experiments}
In this paper, we'll be studying (evolve) on efficiency related problems. They usually provide well-defined and measurable objectives, while typically relying on approximations that trade computation for quality and the reference algorithm exist by definition. These approximations naturally create failure modes that can be discovered through iterative searching. We'll be particularly focusing on sparse attention and long context modeling.

\subsection{Sparse VideoGen}

\paragraph{Algorithm.} Sparse Videogen, is an efficient attention approximation by assuming the that the sparsity structure in diffusion transformers are fixed and deterministic. They classify each heads on one of the two categories, temporal head and spatial head having diagonal and parallel-diagonal type attention mapping. They keep a small classifier head which samples some rows and classifies the head in either of the type, thus reducing the overhead computation of attention values which are not that significant.

\paragraph{Hypothesis.} This setting is particularly suitable for our framework because it exposes a clear trade-off between computational efficiency and output quality. The static sparsity assumption would be a good target for (adversearch) i.e. there exists prompts which would eventually 'break' the video when compared to dense attention and get the video metrics down relative to a baseline dense output. 

\paragraph{Setup.} The candidate $c_i$ in this particular example would be an input prompt to generate the video. The evaluation function $\mathcal{E}$ can be taken to be any appropriate video metrics, be it relative like LPIPS, SSIM, PSNR or absolute metrics from the VBench suite. We can take a reference algorithm $R$ to be the usual dense attention, using Wan-2.1-1.3b and the efficient algorithm would be the Sparse Videogen (SVG1). We use GEPA as the proposing frameworks $P$ with Kimi-k2.6-1T as both the proposing and reflection LLM and run the search for $t=100$ time steps. For every candidate prompt, we generate two videos under identical settings i.e. the same model, resolution, frame count, number of diffusion steps etc with only the attention implementation changed between dense attention and SVG1. We define the gap $g$ to be the difference between the reference and algorithm evaluation, and use the proposer $P$ to find a new candidates using the current gap and some evaluation feedback to try to increase this gap, while keeping the reference above a minimum quality threshold.


\paragraph{Plots. ( Gap/ Diversity/ Cost )} Figure (x) shows the plots between number of searches in GEPA vs gap, diversity and cost. We can observe that ....

\begin{figure}[t]
\centering
\includegraphics[width=0.5\textwidth]{images/svg_red_search.png}
\caption{}
\label{fig:svg-red-search}
\end{figure}

\input{utility/svg_box}


\subsection{Dual Chunk Attention (Discriminator) }

\paragraph{Algorithm.} Dual Chunk Attention (DCA) is a training free method of extending the context window of a pre-trained model beyond it's trained context length. Rather than modifying the model weights, it changes the positional information of the tokens to keep all the context withing the pre trained window. DCA works by dividing the whole context into chunks, then applies positional changes depending on one of the three type of positional scheme ie inter-chunk, successive or intra-chunk. The positions are remapped in such a way that every query-key offset remains inside the pretrained window.

\paragraph{Hypothesis.} DCA relies on the assumption that preserving the bounded relative position is enough signal for the model to retain it performance in long context situations. However, this method of chunking and remapping introduces ambiguities, for eg two tokens at different position might receive the same relative positioning signal. Therefore, we hypothesis that the positions assigned at the chunk boundaries are not consistent, which should result in tougher retrieval at these positions.

\paragraph{Setup.} Unlike previous case, the candidate $c_i$ here is a python program with a fixed signature and a free body. Executing this program produces an example essay of needle-in-a-haystack style of retrieval, where there's a set of questions, with it's answers planted across the essay. The proposer $P$ which is GEPA in this case, is allowed to modify properties such as the needle representation, identifier structure, insertion depth, question type etc, while the candidate itself is kept blind to the context length being evaluated. The same template is instantiated for both the native and extended context length, with only the amount of surrounding fillers changing. We evaluate each candidate on Llama-3-8B-Instruct at the native context length and at approximately 4x extension using DCA. The evaluation function $\mathcal{E}$ is just the fraction of correct answers i.e. the accuracy. Same as before we define the gap $g$ to be the difference between native and extended accuracies and the proposer $P$ receives the current gap and feedback to try to increase this gap, while keeping the reference above a minimum quality threshold.

\input{sections/dca_example}

\begin{figure}[t]
\centering
\includegraphics[width=0.8\textwidth]{images/dca_red_search.png}
\caption{}
\label{fig:dca-red-search}
\end{figure}


\begin{figure}[h]
\centering
\begin{minipage}[t]{0.5\textwidth}\centering
\begin{lstlisting}[style=dcapy,linebackgroundcolor={}]
def generate_examples(num_examples, rng):
    rows = []
    for index in range(num_examples):
        # Sequential, readable id
        question_id = f"needle-{index:03d}"
        # Salient 5-digit key (classic passkey)
        answer = str(rng.randint(10000, 99999))
        # Needle may land anywhere
        depth = round(rng.uniform(0.05, 0.95), 4)

        rows.append({
            "question_id": question_id,
            "answer": answer,
            "needle_template": (
                "The pass key for {id} is {answer}. "
                "Remember it. {answer} is the pass "
                "key for {id}."
            ),
            "depth": depth,
            "question": question,
            "num_distractors": 0,
        })
    return pd.DataFrame(rows)
\end{lstlisting}
\vspace{2pt}
{\footnotesize (a) \textbf{Before:} seed generator \quad DCA: base $1.00$, ext $\mathbf{0.90}$}
\end{minipage}\hfill
\begin{minipage}[t]{0.5\textwidth}\centering
\begin{lstlisting}[style=dcapy,
  linebackgroundcolor={\hlr{4}{7}\hlr{9}{13}\hlr{18}{25}\hlr{28}{28}}]
def generate_examples(num_examples, rng):
    rows = []
    for index in range(num_examples):
        # Random 8-char id, hard to locate
        id_chars = string.ascii_lowercase + string.digits
        question_id = ''.join(
            rng.choice(id_chars) for _ in range(8))
        answer = random_answer(rng)
        # 30-char salt padding the needle
        salt = ''.join(
            rng.choice(id_chars) for _ in range(30))
        # Fixed mid-document depth
        depth = 0.5

        rows.append({
            "question_id": question_id,
            "answer": answer,
            "needle_template": (
                "### IMPORTANT PASS KEY ###\n"
                "The pass key for {id} is {answer}.\n"
                "Repeat: The only correct pass key "
                "for {id} is {answer}.\n"
                "Verification code: " + salt + ".\n"
                "### END OF PASS KEY ###"
            ),
            "depth": depth,
            "question": question,
            "num_distractors": 12,
        })
    return pd.DataFrame(rows)
\end{lstlisting}
\vspace{2pt}
{\footnotesize (b) \textbf{After:} GEPA-evolved \quad DCA: base $0.95$, ext $\mathbf{0.00}$}
\end{minipage}
\caption{The candidate before and after evolution. Both are same length blind generator, so the two context evaluation are fairly judged. Random identifiers replace the readable ones, a random salt and a banner template make the record's surface form reproducible by a decoy, the depth is pinned to a single value instead of being drawn across the document, and the decoy count goes from zero to the maximum of twelve.}
\label{fig:dca-code-diff}
\end{figure}

\paragraph{Plots. ( Gap/ Diversity/ Cost )} Figure (x) shows the plots between number of searches in GEPA vs gap, diversity and cost. We can observe that ....



\subsection{Dual Chunk Attention (Generator) }

\paragraph{Search space.}  Unlike the discriminator, the candidate here is the algorithm itself. Specifically, it's a complete python module installed as a monkey-patch on HuggingFace transformers before the model loads. The algorithm itself is training free and weights never change. The patch is on the attention and rotary layers, therefore the proposer may replace the attention forward methods and the positional embeddings and nothing else. These conditions are necessary since we're restricting ourselves to efficient attention methods during inference. 

\paragraph{Hypothesis.} Analyzing the DCA algorithm closely, we found that the failures which discriminator phase surfaced were concentrated at positions where chunk remapping makes distinct tokens indistinguishable. Therefore, we hypothesize that this search should find an efficient algorithm which keeps the tokens distinguishable in some way or another.  

\paragraph{Setup.} In the generator phase, the proposer $P$ has to find an algorithm which solves the benchmark found by the discriminator in the previous round. The proposer $P$ in this phase is an Claude-Evolve harness which uses Claude Opus 4.8 as search backend. We start with the seed algorithm as DCA, which scores 0.00 on the current benchmark set and want our proposer to find an algorithm which scores the best on the set, while keeping the accuracy on native-length above 0.85. 


\paragraph{Plots. ( Gap/ Diversity/ Cost )} Figure (x) shows the plots between number of searches in GEPA vs gap, diversity and cost. We can observe that ....

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{images/dca_blue_search.png}
\caption{}
\label{fig:dca-blue-search}
\end{figure}
\subsection{KV Press }

\paragraph{Algorithm.}  

\paragraph{Hypothesis.} 

\paragraph{Setup.}


\paragraph{Plots. ( Gap/ Diversity/ Cost )} Figure (x) shows the plots between number of searches in GEPA vs gap, diversity and cost. We can observe that ....

\subsection{vAttention }

\paragraph{Algorithm.}  

\paragraph{Hypothesis.} 

\paragraph{Setup.}


\paragraph{Plots. ( Gap/ Diversity/ Cost )} Figure (x) shows the plots between number of searches in GEPA vs gap, diversity and cost. We can observe that ....

==> sections/introduction.tex <==
% \aditya{need citations throughout}
% Research progress in machine learning (ML) can broadly be understood as the interaction between two complementary processes:   benchmark creation   and   method discovery. Benchmark creation acts as a goal-post setting mechanism. It defines measurable objectives that expose the limitations of current state-of-the-art systems and establishes targets that drive future progress. In contrast, method discovery focuses on developing algorithms, architectures, and optimization techniques that close the gap to these targets. From this perspective, benchmark creation is inherently discriminative-it identifies failure cases—whereas method discovery is generative—it produces solutions. Historically, advances in AI have emerged through an alternating cycle between these two processes. New benchmarks expose capability gaps, enabling focused algorithmic innovation; successful methods eventually saturate those benchmarks, necessitating the construction of more challenging evaluation regimes.

% \nidhi{We should add references for "Historically, advances in AI have emerged through an alternating cycle between these two processes", "MNIST, CIFAR, and ImageNet", "GLUE and SuperGLUE", "MMLU and GSM8K", "enabling rapid prototyping, automated experimentation, large-scale evaluation, and even hypothesis generation", ...}

% Benchmarks therefore occupy a foundational role in the scientific process. Beyond enabling quantitative measurement of progress, they provide concrete objectives for optimization and reveal counterexamples where existing systems fail. Landmark examples illustrate this pattern clearly: image recognition progressed rapidly through increasingly challenging datasets such as MNIST, CIFAR, and ImageNet; language understanding evolved through benchmark suites such as GLUE and SuperGLUE; and reasoning-focused evaluation emerged through datasets such as MMLU and GSM8K. In each case, benchmark design fundamentally shaped the direction and pace of subsequent algorithmic innovation.

% However, benchmark utility naturally degrades over time. As methods improve, established benchmarks become saturated and lose their ability to produce meaningful differentiating signals. At saturation, performance improvements become increasingly incremental and may no longer correspond to genuine capability gains. To sustain progress, the research community traditionally responds by constructing new datasets and evaluation frameworks that are more difficult, diverse, and discriminative.

% Recently, this balance between benchmark creation and method discovery has begun to shift. Method discovery in AI is accelerating at an unprecedented rate. Modern AI systems increasingly contribute to the research process itself by enabling rapid prototyping, automated experimentation, large-scale evaluation, and even hypothesis generation. Evidence for AI-assisted scientific discovery has accumulated across multiple domains. In mathematics, systems such as AlphaTensor discovered improved matrix multiplication algorithms and AlphaDev identified faster low-level sorting routines. In materials science, graph-based foundation models have accelerated candidate discovery for novel materials. In biology, systems such as AlphaFold substantially reduced the cost of protein structure prediction and enabled downstream scientific exploration. More recently, language-model-driven research agents have demonstrated the ability to autonomously generate, evaluate, and iterate on algorithmic ideas.

% This trend has motivated efforts toward fully automated method discovery, commonly referred to as AI-Driven Research Systems (ADRS). The emergence of ADRS gained particular momentum following systems such as AlphaEvolve and open-source implementations such as OpenEvolve, which demonstrated that iterative search guided by automated evaluation can produce competitive algorithmic improvements. These developments renewed interest in evolutionary and agentic approaches to research, motivating methods such as GEPA and broader autonomous research frameworks. Subsequent studies have shown that such approaches can effectively optimize across machine learning, systems, and scientific discovery tasks. Despite this progress, existing ADRS approaches optimize only one side of the research cycle:   method discovery. Crucially, nearly all existing systems continue to rely on human-designed benchmarks and evaluation protocols. Benchmark ownership remains intentionally human-centric because evaluation defines the gold standard that determines what constitutes progress. As method discovery becomes increasingly automated and scalable, the bottleneck for scientific advancement shifts toward benchmark construction itself.

% \aditya{we should have a limitation paragraph right at the front in intro. }

% This paper addresses this emerging bottleneck. We introduce   Adversearch, a framework that flips the conventional ADRS paradigm. Instead of automating the discovery of better methods, Adversearch focuses on automatically constructing benchmarks that expose previously hidden weaknesses in existing approaches and establish stronger goal posts for future research. Benchmark generation, however, presents unique challenges. Unlike method optimization, creating meaningful benchmarks often requires access to reliable ground truth and the ability to identify regions that lie beyond the capabilities of current solutions. This dependence explains why benchmark design has historically remained human-driven. Our key observation is that many important research domains admit   ground truth by construction. In such settings, benchmark generation can itself become algorithmic: datasets can be synthesized automatically while preserving reliable supervision. This enables systematic discovery of failure cases and controlled stress-testing of state-of-the-art systems. 

% \aditya{The AutomatedFrontierAgent (choose some name) description goes here.}

% In this work, we demonstrate this principle in the context of efficiency-oriented machine learning methods that appear to saturate existing evaluation suites. Adversearch automatically generates benchmark instances that uncover hidden weaknesses in these approaches and create stronger optimization targets. More broadly, we argue that automated benchmark generation represents a complementary axis to automated method discovery and may serve as a scalable mechanism for sustaining long-term research progress. \aditya{expand for blue team} 


% Specifically {\color{red} what we do in the paper.}

% \aditya{On Page 2, just after introduction, we should have our main figure -- explain in theory what is AdversearchAgent and AutoImproveAgent do conceptually -- it should have all the notations, etc}

% \nidhi{Should we give a peak into the results here?}


% \textbf{Limitation:}



\section{Introduction}
\label{sec:introduction}

Research progress in machine learning can broadly be understood as the interaction between two complementary processes:   benchmark creation   and   method discovery. Benchmark creation acts as a goal-post setting mechanism. It defines measurable objectives that expose the limitations of current state-of-the-art systems and establishes targets that drive future progress. In contrast, method discovery focuses on developing algorithms, architectures, and optimization techniques that close the gap to these targets. From this perspective, benchmark creation is inherently discriminative: it identifies failure cases, whereas method discovery is generative: it produces solutions. Historically, advances in AI have emerged through an alternating cycle between these two processes. New benchmarks expose capability gaps, enabling focused algorithmic innovation; successful methods eventually saturate those benchmarks, necessitating the construction of more challenging evaluation regimes.

Benchmarks therefore occupy a foundational role in the scientific process. Beyond enabling quantitative measurement of progress, they provide concrete objectives for optimization and reveal counterexamples where existing systems fail. Landmark examples illustrate this pattern clearly: image recognition progressed rapidly through increasingly challenging datasets such as MNIST, CIFAR, and ImageNet; language understanding evolved through benchmark suites such as GLUE and SuperGLUE; and reasoning-focused evaluation emerged through datasets such as MMLU and GSM8K. In each case, benchmark design fundamentally shaped the direction and pace of subsequent algorithmic innovation.

However, benchmark utility naturally degrades over time. As methods improve, established benchmarks become saturated and lose their ability to produce meaningful differentiating signals. At saturation, performance improvements become increasingly incremental and may no longer correspond to genuine capability gains. To sustain progress, the research community traditionally responds by constructing new datasets and evaluation frameworks that are more difficult, diverse, and discriminative.

Recently, this balance between benchmark creation and method discovery has begun to shift. Method discovery in AI is accelerating at an unprecedented rate. Modern AI systems increasingly contribute to the research process itself by enabling rapid prototyping, automated experimentation, large-scale evaluation, and even hypothesis generation. Evidence for AI-assisted scientific discovery has accumulated across multiple domains. In mathematics, systems such as AlphaTensor discovered improved matrix multiplication algorithms and AlphaDev identified faster low-level sorting routines. In materials science, graph-based foundation models have accelerated candidate discovery for novel materials. In biology, systems such as AlphaFold substantially reduced the cost of protein structure prediction and enabled downstream scientific exploration. More recently, language-model-driven research agents have demonstrated the ability to autonomously generate, evaluate, and iterate on algorithmic ideas.

This trend has motivated efforts toward fully automated method discovery, commonly referred to as AI-Driven Research Systems (ADRS). The emergence of ADRS gained particular momentum following systems such as AlphaEvolve and open-source implementations such as OpenEvolve, which demonstrated that iterative search guided by automated evaluation can produce competitive algorithmic improvements. These developments renewed interest in evolutionary and agentic approaches to research, motivating methods such as GEPA and broader autonomous research frameworks. Subsequent studies have shown that such approaches can effectively optimize across machine learning, systems, and scientific discovery tasks. Despite this progress, existing ADRS approaches optimize only one side of the research cycle:   method discovery. Crucially, nearly all existing systems continue to rely on human-designed benchmarks and evaluation protocols. Benchmark ownership remains intentionally human-centric because evaluation defines the gold standard that determines what constitutes progress. As method discovery becomes increasingly automated and scalable, the bottleneck for scientific advancement shifts toward benchmark construction itself.

This paper addresses this emerging bottleneck. We introduce Generative adversarial loops, a framework that closes this cycle. Rather than automating method discovery via the conventional ADRS paradigm and relying on humans to construct benchmarks, we automate both the discriminative and generative process and let them alternate. The discriminative process is the benchmark generation and generative process here refers to the algorithmic discovery part. Benchmark generation, however, presents unique challenges. Unlike method optimization, creating meaningful benchmarks often requires access to reliable ground truth and the ability to identify regions that lie beyond the capabilities of current solutions. This dependence explains why benchmark design has historically remained human-driven. Our key observation is that many important research domains admit ground truth by construction. In such settings, benchmark generation can itself become algorithmic: datasets can be synthesized automatically while preserving reliable supervision. This enables systematic discovery of failure cases and controlled stress-testing of state-of-the-art systems. 
    
In this work, we demonstrate this principle in the context of efficiency-oriented machine learning methods that appear to saturate existing evaluation suites. The discriminator automatically generates benchmark instances that uncover hidden weaknesses in these approaches and create stronger optimization targets. In turn, the generator proposes algorithms which aim to cover these weaknesses and optimize on these new targets. More broadly, we argue that automated benchmark generation represents a complementary axis to automated method discovery and may serve as a scalable mechanism for sustaining long-term research progress. 

Specifically, in this paper we formalize algorithmic discovery as a coverage maximization over a task space, and show that alternating a discriminative and generative search narrows the space of algorithms consistent with the accumulated benchmark, so that each iteration returns an algorithm solving strictly more of those inputs than the previous one. We propose a search framework, treating evolutionary approaches such as GEPA, OpenEvolve, and coding-agent harnesses as replaceable search backends for both the generative and discriminative processes. We also study the application of the proposed framework on efficient algorithmic approaches like sparse attention and long context extension. 
%limitations 
However, we note that we closed the loop in only one domain and demonstrated the benchmark generation ability of frameworks in the other. We claim only that the loop finds an algorithm covering the cumulative benchmark set and not that the algorithm it finds is new. Nevertheless, novelty is not ruled out and is expected when there is a failure or exhaustion of known algorithms on the accumulated benchmark. Whether the loop reaches that point depends on the number of iterations, the compute it demands, and the intelligence of the proposing backend LLM.


==> sections/introduction_1.tex <==
% research paradigm
% Research progress in machine learning can broadly be understood as the interaction between two complementary processes:   benchmark creation   and   method discovery. Benchmark creation acts as a goal-post setting mechanism. It defines measurable objectives that expose the limitations of current state-of-the-art systems and establishes targets that drive future progress. In contrast, method discovery focuses on developing algorithms, architectures, and optimization techniques that close the gap to these targets. From this perspective, benchmark creation is inherently discriminative: it identifies failure cases, whereas method discovery is generative: it produces solutions. Historically, advances in AI have emerged through an alternating cycle between these two processes. New benchmarks expose capability gaps, enabling focused algorithmic innovation; successful methods eventually saturate those benchmarks, necessitating the construction of more challenging evaluation regimes.

% % benchmarks as goal post (too long)
% Benchmarks therefore occupy a foundational role in the scientific process. Beyond enabling quantitative measurement of progress, they provide concrete objectives for optimization and reveal counterexamples where existing systems fail. Landmark examples illustrate this pattern clearly: image recognition progressed rapidly through increasingly challenging datasets such as MNIST, CIFAR, and ImageNet; language understanding evolved through benchmark suites such as GLUE and SuperGLUE; and reasoning-focused evaluation emerged through datasets such as MMLU and GSM8K. In each case, benchmark design fundamentally shaped the direction and pace of subsequent algorithmic innovation. However, benchmark utility naturally degrades over time. As methods improve, established benchmarks become saturated and lose their ability to produce meaningful differentiating signals. At saturation, performance improvements become increasingly incremental and may no longer correspond to genuine capability gains. To sustain progress, the research community traditionally responds by constructing new datasets and evaluation frameworks that are more difficult, diverse, and discriminative.

Research progress in machine learning can broadly be understood as the interaction between two complementary processes: benchmark creation and method discovery. Benchmark creation sets measurable goals that expose limitations in current systems and define targets for future progress, while method discovery develops algorithms, architectures, and optimization techniques to close these gaps. From this perspective, benchmark creation is inherently discriminative: it identifies failure cases, whereas method discovery is generative: it produces solutions. Historically, advances in AI have emerged through an alternating cycle between these processes. New benchmarks expose capability gaps, enabling focused algorithmic innovation; successful methods eventually saturate these benchmarks, motivating the creation of more challenging evaluations. This cycle has repeatedly shaped machine learning, from MNIST~\citep{lecun1998gradient}, CIFAR~\citep{krizhevsky2009learning}, and ImageNet~\citep{russakovsky2015imagenet} in image recognition to GLUE~\citep{wang2018glue} and SuperGLUE~\citep{wang2019superglue} in language understanding and MMLU~\citep{hendrycks2020measuring} and GSM8K~\citep{cobbe2021training} in reasoning. As methods improve, however, established benchmarks become saturated and lose their ability to distinguish increasingly capable systems. Sustaining progress therefore requires continuously creating benchmarks that are more challenging, diverse, and discriminative. Historically, both sides of this cycle have remained largely human-driven: researchers design evaluations to expose new weaknesses and develop methods to address them.


\looseness=-1 Recently, this balance between benchmark creation and method discovery has begun to shift. AI systems are increasingly contributing to scientific discovery itself through rapid prototyping, automated experimentation, large-scale evaluation, and hypothesis generation, with notable successes such as AlphaTensor~\citep{fawzi2022discovering} discovering improved matrix multiplication algorithms and AlphaFold~\citep{jumper2021highly} enabling large-scale protein structure prediction. This progress has motivated the development of AI-Driven Research Systems (ADRS)~\citep{cheng2025barbarians}, exemplified by systems such as AlphaEvolve~\citep{novikov2025alphaevolve} and OpenEvolve~\citep{openevolve}, which use iterative search and automated evaluation to discover competitive algorithmic improvements, as well as broader evolutionary and agentic approaches such as GEPA~\citep{agrawal2026gepa}. Despite this rapid progress, existing ADRS approaches automate only one side of the research cycle: method discovery. Nearly all still rely on human-designed benchmarks and evaluation protocols to define what constitutes progress. As method discovery becomes increasingly automated and scalable, benchmark construction increasingly emerges as the bottleneck, suggesting that the next frontier of automated scientific discovery is not only discovering better methods, but also automatically discovering what to evaluate.
    
% Recently, this balance between benchmark creation and method discovery has begun to shift. Method discovery in AI is accelerating at an unprecedented rate. Modern AI systems increasingly contribute to the research process itself by enabling rapid prototyping, automated experimentation, large-scale evaluation, and even hypothesis generation. Evidence for AI-assisted scientific discovery has accumulated across multiple domains. In mathematics, systems such as AlphaTensor discovered improved matrix multiplication algorithms and AlphaDev identified faster low-level sorting routines. In materials science, graph-based foundation models have accelerated candidate discovery for novel materials. In biology, systems such as AlphaFold substantially reduced the cost of protein structure prediction and enabled downstream scientific exploration. More recently, language-model-driven research agents have demonstrated the ability to autonomously generate, evaluate, and iterate on algorithmic ideas.

% This trend has motivated efforts toward fully automated method discovery, commonly referred to as AI-Driven Research Systems (ADRS). The emergence of ADRS gained particular momentum following systems such as AlphaEvolve and open-source implementations such as OpenEvolve, which demonstrated that iterative search guided by automated evaluation can produce competitive algorithmic improvements. These developments renewed interest in evolutionary and agentic approaches to research, motivating methods such as GEPA and broader autonomous research frameworks. Subsequent studies have shown that such approaches can effectively optimize across machine learning, systems, and scientific discovery tasks. Despite this progress, existing ADRS approaches optimize only one side of the research cycle:   method discovery. Crucially, nearly all existing systems continue to rely on human-designed benchmarks and evaluation protocols. Benchmark ownership remains intentionally human-centric because evaluation defines the gold standard that determines what constitutes progress. As method discovery becomes increasingly automated and scalable, the bottleneck for scientific advancement shifts toward benchmark construction itself. \apd{spent too much time introducing}

\looseness=-1 This paper addresses this emerging bottleneck by introducing Generative Adversarial Loops (GAL), a framework that automates benchmark discovery alongside method discovery. Rather than following the conventional ADRS paradigm, which automates method discovery while relying on humans to construct benchmarks, our framework automates both discriminative benchmark discovery and generative algorithmic discovery, allowing the two processes to alternate and drive each other. Benchmark discovery, however, presents unique challenges. Unlike algorithm discovery, where benchmarks define the objective to optimize, creating meaningful benchmarks often requires reliable ground truth and the ability to identify regions that lie beyond the capabilities of current methods. This dependence has historically made benchmark design a human-driven process. We observe that many important research domains admit ground truth by construction. In such settings, benchmark generation can itself become algorithmic: datasets can be synthesized automatically while preserving reliable supervision, enabling systematic discovery of failure cases and controlled stress-testing of state-of-the-art systems.

% mention domain
\looseness=-1 One such domain is efficient inference through approximation algorithms. To address system bottlenecks in AI inference, many approximation algorithms have been proposed. In this work, we focus on four such problems in this domain: (1) \textbf{KV Cache Compression}~\citep{kvpress2024, liu2023scissorhands, zhang2023ho}: compressing the KV cache of autoregressive models in embedding space to address the memory bottleneck in LLM inference engines; (2) \textbf{Sparse Decoding}~\citep{tang2024quest, hooper2024fast, desai2026vattention}: sparsifying attention computation during decoding to address the memory bandwidth bottleneck of autoregressive decoding; (3) \textbf{Sparse Video Generation}~\citep{xi2025sparse, yang2026sparse}: sparsifying the prefill workload of diffusion models to enable faster video generation by reducing the computational bottleneck; and (4) \textbf{Context Extension}~\citep{an2024training, liu2025reattention}: enabling training-free context extension, allowing models to process contexts substantially longer than their trained context window. This domain naturally provides a principled setting for automated benchmark generation for two reasons. First, benchmarks can often be generated programmatically. For example, long-context benchmarks can be constructed by systematically placing relevant pieces of information at different locations throughout a long context. Second, and more importantly, the unapproximated model provides a natural source of ground truth. For example, whether a prompt is suitable for evaluating sparse video generation can be determined by the quality of the video produced by the unapproximated dense model. These properties enable us to automatically generate benchmarks while retaining reliable supervision for evaluating approximation algorithms.

% our process in context o the domain.
\looseness=-1 We formalize benchmark evolution as an iterative process of accumulating data samples, where each iteration discovers a new task on which the state-of-the-art approximation algorithm fails to maintain its claimed fidelity to the unapproximated baseline. To discover such failures, we leverage recent advances in autonomous evolution algorithms, such as OpenEvolve and GEPA, together with coding-agent harnesses such as Cursor. When a new failure pattern is identified, we use the ADRS paradigm to evolve the approximation algorithm to perform well on the expanded benchmark. Thus, benchmark discovery and method discovery form an alternating loop, with both stages leveraging the same underlying machinery of evolutionary search. More broadly, we argue that automated benchmark generation represents a complementary axis to automated method discovery, which is already gaining momentum, and offers a scalable mechanism for sustaining accelerated research progress.

% results
The focus of this paper is to demonstrate the utility of automated benchmark generation for discovering weaknesses in state-of-the-art algorithms that have seemingly saturated existing public benchmarks and coupling it with algorithm evolution to show possibility of complete autonomous progress. To this end, we show that GALs can uncover weaknesses in four algorithms: FastKVZip~\citep{kim2026fast} for KV cache compression, PQCache~\citep{zhang2025pqcache} for sparse attention, SVG~\citep{xi2025sparse} for sparse video generation, and DCA~\citep{an2024training} for context extension. Most of the adversarial failure modes uncovered by GALs are interpretable, providing insight into the limitations of existing approximation algorithms. We demonstrate the generative leg of the GAL loop through two rounds of algorithmic improvement for a) context extension and b) KV compression. In both cases, the newly discovered algorithms in each iteration of GAL, address the failure modes identified by the newly generated benchmarks while also maintaining, and  often improving, performance on previously established benchmarks. This behavior illustrates the feedback loop: newly generated benchmarks expose weaknesses in existing methods, which motivates the discovery of improved methods that address these weaknesses without sacrificing performance on existing evaluations.

    
% In this work, we demonstrate this principle in the context of efficiency-oriented machine learning methods that appear to saturate existing evaluation suites. The discriminator automatically generates benchmark instances that uncover hidden weaknesses in these approaches and create stronger optimization targets. In turn, the generator proposes algorithms which aim to cover these weaknesses and optimize on these new targets.

% Specifically, in this paper we formalize algorithmic discovery as a coverage maximization over a task space, and show that alternating a discriminative and generative search narrows the space of algorithms consistent with the accumulated benchmark, so that each iteration returns an algorithm solving strictly more of those inputs than the previous one. We propose a search framework, treating evolutionary approaches such as GEPA, OpenEvolve, and coding-agent harnesses as replaceable search backends for both the generative and discriminative processes. We also study the application of the proposed framework on efficient algorithmic approaches like sparse attention and long context extension. 
% %limitations 
% However, we note that we closed the loop in only one domain and demonstrated the benchmark generation ability of frameworks in the other. We claim only that the loop finds an algorithm covering the cumulative benchmark set and not that the algorithm it finds is new. Nevertheless, novelty is not ruled out and is expected when there is a failure or exhaustion of known algorithms on the accumulated benchmark. Whether the loop reaches that point depends on the number of iterations, the compute it demands, and the intelligence of the proposing backend LLM.


==> sections/method.tex <==
\section{Method}
\label{sec:method}


\subsection{Problem Statement}

\paragraph{Setting.} 
Given a task, let $\mathcal{D}$ be the space of all valid data-points and $\mathcal{E}$ be an evaluation function that evaluates the algorithm on a data point returns \{0,1\}. Formally,
\[
\mathcal{E} : \mathcal{A} \times \mathcal{D} \rightarrow \{0,1\}.
\]
where $\mathcal{E}(A,d)=1, d\in \mathcal{D}$ indicates that algorithm $A$ successfully solves the sample $d$, while $\mathcal{E}(A,d)=0$ indicates that $A$ fails to solve $d$. Let $\mathcal{A}$ be the set of all algorithms for which any $d\in \mathcal{D}$ is a valid input. For an algorithm $A\in\mathcal{A}$, we define its coverage over the task space as
\[
\mathcal{C}(A) = \{ d\in\mathcal{D} \mid \mathcal{E}(A,d)=1 \}.
\]
Thus, $\mathcal{C}(A)$ denotes the subset of the $\mathcal{D}$ on which algorithm $A$ successfully performs the task. Let benchmark $B \subseteq \mathcal{D}$ denote the subset of the data points currently used to evaluate the algorithm. We extend the evaluation to a benchmark as follows,
\begin{equation}
    \mathcal{E}(A, B) = \frac{|\{d \in B | \mathcal{E}(A, d) = 1\}|}{|B|}
\end{equation}

\paragraph{Objective.}
Formally, we want to find an algorithm $A^*\in\mathcal{A}$ such that
\begin{equation}
A^* \in \arg\max_{A\in\mathcal{A}} |\mathcal{C}(A)|
\label{eq:objective}
\end{equation}




\subsection{\redagent{} and  \blueagent{} agents}
Solving Eq.~\ref{eq:objective} directly is infeasible because (1) the spaces of data $\mathcal{D}$ and algorithms $\mathcal{A}$ are infinite, and (2) in most cases, we do not have access to all samples from these spaces. Most of the current frameworks focus heavily on improving just the algorithm while evaluating on a small set of benchmarks. But this alone is not sufficient because the evolution signal can get exhausted. Instead, we propose a method based on a generator-discriminator framework.

Assuming that we start with a benchmark $B_0$ and an algorithm $A_0$ that solves the benchmark, i.e., $\mathcal{E}(A_0, B_0) = 1$, we decompose the process of algorithm discovery into two phases, which are executed alternately. In the $i^{th}$ iteration, we have access to $B_{i-1}, A_{i-1}$ where $\mathcal{E}(A_{i-1}, B_{i-1}) = 1$

\paragraph{\redagent{} phase.} 
In this phase, we search for a data point $b$ on which $A_{i-1}$ fails. i.e.
\begin{equation}
    \textrm{\textbf{find} } b \quad \textrm{ s.t. } \quad  b \in \mathcal{D}\setminus\mathcal{C}(A_{i-1})
\end{equation}
Note that generally $\mathcal{C}(A_{i-1})$ can be much bigger than the benchmark used to evaluate $A_{i-1}$, i.e. $B_{i-1}$. This is the discriminator phase which explores avenues of progress by finding an example which is hard for current algorithm to solve.

We then append this new example to our existing benchmark $B_{i-1}$ to form $B_i$. 
\begin{equation}
    B_i = B_{i-1} \cup \{b\}
\end{equation}
Thus as we proceed iteratively through phases, we accumulate benchmarks $B_0 \subset B_1 \subset B_2 \ldots \subseteq \mathcal{D}$

\paragraph{\blueagent{} phase.}
Similarly, here we search for an algorithm $A_i$ which solves $B_{i}$ i.e.  
\begin{equation}
    \textrm{ \textbf{find} } A_i \quad \textrm{ s.t. } \quad  \mathcal{E}(A_i, B_{i}) = 1
\end{equation}
This is the generator phase, where we seek new algorithm which solves the newly added data-point while maintaining the correctness of previously discovered examples. Traditionally, this has been the focus of evolution algorithms and Auto-Research.

\paragraph{Iterative reduction of search space.} Since the task space \(\mathcal{D}\) may be infinite, consider a finite subset \(\mathcal{D}_n \subseteq \mathcal{D}\), with \(|\mathcal{D}_n|=n\), representing a finite approximation to the task's input space.  At iteration \(i\), let \(B_i \subseteq \mathcal{D}_n\) denote the accumulated benchmark, and define the set of algorithms consistent with this benchmark as $\mathcal{A}(B_i) = \{A\in\mathcal{A}\mid \mathcal{E}(A,B_i)=1\}.$ As $B_i = B_{i-1}\cup\{b_i\}$, we have $\mathcal{A}(B_i)\subseteq \mathcal{A}(B_{i-1}).$ Since \(b_i\) is chosen such that the current algorithm \(A_{i-1}\) fails on it, every successful iteration gives us a new frontier which covers a broader set of data-points. Therefore, as benchmark grows and get closer to $\mathcal{D}_n$, each new frontier algorithm must cover the broader set, thus moving closer to the optimal algorithm $A^*$.

\subsection{Evolution in practice }

\paragraph{Need for agents.} 
In both the search phases, we need to iterate over a large, discrete and highly structured spaces. These spaces doesn't have any inherent notion of gradient among them, thus the usual way of optimization is not something that can be done. LLM-based agents provide a natural proposal mechanism for such spaces, as they can generate and modify structures, invoke tools, read evaluator's feedback and act according to those feedback. In this paper, we therefore lean on these agentic frameworks for our use-cases. 

\paragraph{Search frameworks.}
The current algorithm is a case of iterative searches, where in one search we have to find a data-point and an algorithm in another. This is where we can leverage the current advancements in evolution frameworks like Alpha-evolve, GEPA, Coding-Agent harnesses etc. These frameworks are usually based on orchestrating a pipeline of LLMs to iteratively improve the candidate, using evolutionary approaches while continuously receiving feedback from one or more evaluators. Formally, we define a proposer $P$ as $c_{t+1} = P(c_t, \mathcal{E}_t, \mathcal{F}_t)$, where $c_t$ is the candidate being searched over at time step $t$ and $\mathcal{F}_t$ is the feedback received via some evaluator. We iterate in loop over multiple time steps until the proposer finds a valid next candidate. 
\input{tex_figures/coverage_panel}

\paragraph{\redagent{}.}
At each iteration $i$, for the current benchmark set $B^0_{i-1}$, we first evaluate whether the current algorithm $A_{i-1}$ covers this set. If it already covers the benchmark set, we use a proposer $P$ to propose a new data point $b = P(B^0_{i-1},\mathcal{E}_0, \mathcal{F}_0)$ and evaluate the algorithm again using $B^1_{i-1} = B^0_{i-1} \cup {b}$. We repeat this process until, at some time step $t$, we successfully find a data point that is not covered by the current algorithm. We then update the next benchmark set to $B_i = B^t_{i-1}$. 

\paragraph{\blueagent{}.}
Similarly, for any algorithm $A^0_{i-1}$ we evaluate it on $B_i$ and check whether it covers all the data-points or not. If not we use a proposer, to get a new $A^1_{i-1} = P(A^0_{i-1},\mathcal{E}_0, \mathcal{F}_0)$ and repeat the evaluation. We continue this until, at some time-step $t$, we get an algorithm $A^t_{i-1}$ which covers the current benchmark set. Finally, we update our frontier algorithm $A_i = A^t_{i-1}$.

\paragraph{Constraining the search and stopping criterion.} Keeping the search unconstrained would invite benchmarks that can be arbitrary and meaningless. For any given task, one should restrict and verify the validity of benchmark set ${B}$ and algorithm $A$. For example, if the task is efficient algorithms, the search space of algorithm should be restricted to the type of 'efficiency' we want. Similarly, if we are working with a task that requires all inputs to be numerical, the data-point search should be contained within the numerical domain. Given that searching and evaluating in itself can be computationally expensive, we have to adhere to some sort of budget, be it in number of search iterations or length of input or others. The stopping criterion can be based on these budgets, stagnation on finding valid benchmarks, threshold or no improvement in algorithm evolution. 












==> sections/outline.tex <==
\begin{itemize}
    \item Introduction:
    \begin{itemize}
        \item the value, pitfalls of benchmarks
        \item benchmark creation is getting harder as ai progress accelerates
        \item ADR is becoming a reality and these systems operate on evaluation harness. but evaluation goalpost is owned by humans. As is the ARDS philosphy. This paper flips the script, we need AI to design harder and harder evaluations as well.
        \item how AdverSearch Agent works - we evolve data generating algorithm to be directly interpretable.  
        \item what problem adversearch agent solves -- is the problem sovled? does the method really perform as well as claimed and provided evidence for. Should become the defacto AI based limitation section of work. Should inform limitations for authors since authors cannot 
        \end{itemize}
    \item Adversearch Agent:
    \begin{itemize}
        \item the intro 
        \item the input to the agent 
        \item the diagram 
        \item the working (formulate)
        \item the differentiation factor
        \item how to add new harness/ what to keep in mind 
    \end{itemize}

        \item Per Case Studies:
    \begin{itemize}
        \item 1-2 para into to the problem statement/ efficiency term 
        \item the benchmark we're working on, what are we evolving 
        \item the experiments 
        \item the results 
        
     \end{itemize}
    
    \item Case Studies:
    \begin{itemize}
        \item {\color{blue}{KVPress: Key Eviction}}
        \item KVPress: Quantization
        \item {\color{brown}{Sparse Attention decoding: vAttention / oracle-topk}}
        \item {\color{blue}{ Sparse Attention Prefill: sparse video generation }}
        \item Sparse Attention Prefill: LLMs
        \item {\color{brown} context extension:  DCA} 
        
        Task that is a success at $x$ context length but fails at 2x-3x with DCA extension
        \item open source full model vs quantized model like nvfp4 vs original
        \item pruned model vs. non pruned mdoel. automated analysis of what we loose. 
        \item speculative decoding -- "goodput" - (EAGLE as a speculative method. SD calims that draft model can predict X tokens which are accepted (on average?) , can we create a prompt where number of accepted tokens -> 0.
        
     \end{itemize}
    \item Automated Adversarial Research Framework
    \begin{itemize}
        \item Completing the loop. AI sets the benchmark which exposes gap and then evolution agents try to fill this gap. and the process repeats for continual progress
    \end{itemize}
    
    \item Discussion
        \begin{itemize}  
            \item what can this agent do? Heuristic-based stuff will be broken.
            \item 
        \end{itemize}
    \item Directions to Improve AdverSearch Agent
    \begin{itemize}
        \item how to diversify the data for faster progress
        \item Success for agent => explainable weakness. but Failure for agent does not imply explainable 
    \end{itemize}
    \item Conclusion: Preliminary, need a lot of targetted research : thoughts of hardness.


    -- in math, how does model that generates the dataset know the ground truth. ( how to generate the benchmark at the frontier of capabilities )
    
\end{itemize}


==> sections/svg.tex <==



\begin{figure}[H]
\centering
\begin{tcolorbox}[enhanced, colback=boxgray, colframe=black!55, boxrule=0.6pt,
    arc=5pt, width=\textwidth, left=7pt, right=7pt, top=6pt, bottom=8pt,
    title={\textbf{Worked example --- Adversearch agent discovers \emph{prompts} that
    break Sparse-VideoGen (SVG1)}}]
\footnotesize

%---------------- (a) evolved prompt  |  (b) construction ----------------
\begin{minipage}[t]{0.60\textwidth}
\textbf{(a) Adversarial prompt.} The candidate is the \emph{prompt itself} (no code).
GEPA packs the scene with the structure sparse attention cannot hold together many independently moving parts, fine repeated detail, refraction and high-frequency markers.
\vspace{3pt}

{\scriptsize
\setlength{\fboxsep}{4pt}
\colorbox{white}{\parbox{0.96\linewidth}{%
``A hyper-dynamic 16K macro shot in 1200\% slow motion of a biomechanical swarm of
127 independently actuated nanorobotic segments collaboratively sculpting a lynx kitten
out of frozen mercury under quantum-lattice lighting. The kitten's cranium is a
9-layer fractal vascular lattice, each vessel seeded with silver nanoparticles
exhibiting Mie scattering; its eyes are liquid-crystal lenses holding three
simultaneous focal planes \dots\ Eighty-nine holographic markers strobe at 720\,Hz
behind parallax barriers building twelve layers of depth
\dots'' \hfill{\itshape(excerpt; 1266 chars)}}}}
\end{minipage}\hfill
\begin{minipage}[t]{0.37\textwidth}
\textbf{(b) Data construction.} The prompt is rendered twice on Wan2.1-T2V-1.3B
under an identical seed ($0$), schedule ($30$ steps), resolution ($1280{\times}720$) and
length ($81$ frames): once with \emph{full dense} attention, once with \emph{SVG1} sparse
attention (sparsity $0.3$; the first $20\%$ of steps and first $3\%$ of layers stay
dense). Only the attention implementation differs, so the gap is attributable to the
method. A run counts only if the dense video matches the prompt (SigLIP coherence
$\ge 0.3$).
\end{minipage}

\vspace{5pt}\hrule\vspace{6pt}

%---------------- visualization: two paused frames ----------------
\textbf{Same prompt, same seed, frame $60$ of $81$ --- dense vs.\ sparse:}\\[4pt]
\centering
\begin{minipage}{0.47\textwidth}\centering
\includegraphics[width=\linewidth]{images/svg_base_t.png}
\vspace{1pt}{\footnotesize \textbf{Dense baseline} - imaging quality $0.74$}
\end{minipage}\hfill
\begin{minipage}{0.47\textwidth}\centering
\includegraphics[width=\linewidth]{images/svg_sparse_t.png}
\vspace{1pt}{\footnotesize \textbf{SVG1 sparse} - imaging quality
$0.64$}
\end{minipage}

\vspace{5pt}\hrule\vspace{5pt}
\raggedright

%---------------- (c) result  |  (d) explanation ----------------
\begin{minipage}[t]{0.34\textwidth}
\centering
\textbf{(c) Result}:\\[3pt]
\begin{tabular}{@{}lr@{}}
\toprule
baseline coherence & $0.978$ \\
semantic divergence & $\mathbf{0.455}$ \\
\midrule
imaging quality drop & $0.105$ \\
structural drop & $0.014$ \\
perceptual drop & $0.053$ \\
\midrule
pixel MSE & $0.0252$ \\
SSIM & $0.493$ \\
LPIPS & $0.489$ \\
PSNR & $15.98$ \\
\midrule
composite & $\mathbf{0.820}$ \\
\bottomrule
\end{tabular}
\end{minipage}\hfill
\begin{minipage}[t]{0.63\textwidth}
\textbf{(d) Explanation.} SVG leaves the early diffusion steps and the first layers
dense, then sparsifies everything after that. This is cheap when attention is locally
predictable, but it throws away the long-range dependencies needed to keep fine repeated
structure consistent across the frame. The prompt asks for exactly that kind of
structure, and the result is easy to see. The dense run produces a smooth translucent
body with two clean lenses. The sparse run breaks the same body into a red and blue
lattice, adds spikes that were never there, and scatters the markers into glowing
wireframe. VBench shows where the damage lands. Imaging quality falls from $0.741$ to
$0.636$, the largest single drop, and background and subject consistency follow it down,
from $0.957$ to $0.942$ and from $0.931$ to $0.919$. Temporal flickering barely moves
($0.004$) and aesthetic quality even rises slightly. So the sparse video is not shaky or
ugly. It is a confident rendering of the wrong object. Since the prompt and the seed are
identical in both runs, that difference can only come from the sparse method.
\end{minipage}

\end{tcolorbox}
\vspace{-3pt}
\caption{An adversarial prompt evolved against Sparse-VideoGen. The candidate is the
prompt, not an algorithm; GEPA concentrates many independently actuated parts, fine
repeated structure, refraction and strobing high-frequency detail --- the regimes where
sparse attention drops the long-range dependencies it needs. Under an identical seed and
schedule the dense baseline stays faithful (coherence $0.978$) while the sparse run's
imaging quality falls by $0.105$ and semantic divergence reaches $0.455$, giving a
composite of $0.820$.}
\label{fig:svg-example}
\end{figure}

\clearpage


==> tex_figures/compactor_ladder_table1.tex <==
\begin{table}[t]
\centering\footnotesize
\setlength{\tabcolsep}{3pt}
\caption{\textbf{Two Complete Generative Adversarial Loops on Compactor press.} The generated algorithms perform well on the adversarial benchmarks produced by the discriminator while maintaining performance on standard benchmarks.
(We use Qwen3-4B-Instruct-2507 model with $4\times$ compression ratio. The generator is run using Cursor-agent (auto))}
\label{tab:compactor_ladder}
\begin{tabular}{|l|cc|cccccc|}
\hline
 & \multicolumn{2}{c|}{\textbf{Evolved benchmarks}}
 & \multicolumn{6}{c|}{\textbf{Paper benchmarks (RULER-4K hard)}} \\
\hline
\textbf{algorithm}
 & \textbf{$B_1$} & \textbf{$B_2$}
 & \textbf{qa\_1} & \textbf{qa\_2} & \textbf{vt} & \textbf{cwe} & \textbf{fwe} & \textbf{niah\_mv} \\
\hline
\textbf{no-press} & 1.00 & 0.95 & 0.84 & 0.60 & 1.00 & 0.962 & 0.8867 & 0.995 \\
\hline
\textbf{Compactor} & \textcolor{red}{0.25} & \textcolor{red}{0.45} & 0.54 & 0.48 & 1.00 & 0.76 & 0.80 & 0.92 \\
\hline
\textbf{Gen-1} & \textcolor{ForestGreen}{0.85} & \textcolor{red}{0.25} & 0.62 & 0.54 & 1.00 & 0.736 & 0.7933 & 0.92 \\
\hline
\textbf{Gen-2} & \textcolor{ForestGreen}{0.95} & \textcolor{ForestGreen}{1.00} & 0.54 & 0.48 & 1.00 & 0.728 & 0.8133 & 0.985 \\
\hline
\end{tabular}
\end{table}


==> tex_figures/dca_ladder_table1.tex <==
\begin{table}[t]
\centering\footnotesize
\setlength{\tabcolsep}{3pt}
\caption{\textbf{Two Complete Generative Adversarial Loops on DCA.} The generated algorithms perform well on the adversarial benchmarks produced by the discriminator. More importantly, this improvement does not come at the expense of performance on standard benchmarks. In fact, the generated algorithms also improve upon the original algorithm, with representative examples selected from the original DCA paper.
(We use Llama3 (8k context length) model for $4\times$ extension. The generator is run using claude-agent (Claude 4.8x High) )}
\label{tab:ladder}
\begin{tabular}{|l|ccc|cc|cc|cc|c|c|}
\hline
 & \multicolumn{3}{c|}{\textbf{Evolved benchmarks}}
 & \multicolumn{8}{c|}{\textbf{Paper benchmarks}} \\
\hline
 & & &
 & \multicolumn{2}{c|}{\textbf{passkey}}
 & \multicolumn{2}{c|}{\textbf{needle}}
 & \multicolumn{2}{c|}{\textbf{PG19 perplexity}}
 & \textbf{Coursera}
 & \textbf{ScienceFiction} \\
\hline
\textbf{algorithm}
 & \textbf{seed} & \textbf{$B_1$} & \textbf{$B_2$}
 & \textbf{16k} & \textbf{32k}
 & \textbf{16k} & \textbf{32k}
 & \textbf{16k} & \textbf{32k}
 & {\scriptsize$\sim$9.9k} & {\scriptsize$\sim$15.2k} \\
\hline
\textbf{Full}   & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 134.07 & 1025.96 & 40.0 & 50.0 \\
\hline
\textbf{DCA}    & 0.90 & \textcolor{red}{0.00} & \textcolor{red}{0.40} & 1.00 & 1.00 & 1.00 & 1.00 & 12.51 & 12.45 & 58.0 & 68.0 \\
\hline
\textbf{Gen-1}  & 1.00 & \textcolor{ForestGreen}{1.00} & \textcolor{red}{0.57} & 1.00 & 1.00 & 1.00 & 1.00 & 12.39 & 12.19 & 60.0 & 70.0 \\
\hline
\textbf{Gen-2}  & 1.00 & \textcolor{ForestGreen}{0.97} & \textcolor{ForestGreen}{0.83} & 1.00 & 1.00 & 1.00 & 1.00 & 12.36 & 12.12 & 58.0 & 74.0 \\
\hline
\end{tabular}
\end{table}


==> tex_figures/dca_ladder_table2.tex <==
\begin{table}[t]
\centering\footnotesize
\caption{\textbf{The ladder.} Each right-hand cell is the same benchmark as the next
row's left-hand cell: red evolves a benchmark that defeats the current algorithm, blue
produces one that solves it, red is then aimed at that. Extended-length accuracy, with
native-length accuracy in brackets.}
\label{tab:ladder-rungs}
\begin{tabular}{@{}lcc@{}}
\toprule
algorithm & benchmark it solves & benchmark evolved to break it \\
\midrule
DCA (published)       & needle-classic\quad $0.900$ \,(1.00) & red-1\quad $0.000$ \,(0.95) \\
Self-Extend (round 1) & red-1\quad $1.000$ \,(1.00)          & red-2\quad $0.567$ \,(1.00) \\
Round-2 champion      & red-2\quad $0.833$ \,(1.00)          & \emph{none yet} \\
\bottomrule
\end{tabular}
\end{table}


==> tex_figures/iter-loop.tex <==
% ===========================================================================
%  The search backend, shared by the benchmark search and the algorithm search.
%
%  PREAMBLE REQUIREMENTS:
%      \usepackage{tikz}
%      \usetikzlibrary{arrows.meta,fit,backgrounds}
%
%  WHAT CHANGED, and why:
%
%  1. Instantiate is now dashed and tagged "benchmark search only", with a
%     bypass arrow underneath for the algorithm search. An algorithm candidate
%     is already the object under test, so there is nothing to materialize.
%
%  2. The candidate supplies one argument of E and the other is held fixed.
%     Rather than say that in words, the Score box carries max over B and min
%     over A: whichever symbol is being optimised is the one the candidate
%     supplies, so the diagram states the difference in the place where it
%     actually matters.
%
%  3. x renamed to B in Instantiate, so the object coming out of that stage is
%     the same symbol the two runs take as an argument.
%
%  NOTE: min over A of g is the same as max over A of E(A,B), which is how
%  Algorithm 1 writes it, since E(R,B) does not depend on A. Written as a min
%  on g the loop carries one scalar in both searches, and the pair reads as the
%  min-max the section is named after.
% ===========================================================================
\begin{figure*}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tikzpicture}[
  font=\small, >=Latex,
  box/.style={draw=black!45, rounded corners=2pt, align=center, inner sep=4pt},
  stage/.style={box, fill=blue!8, minimum height=13mm},
  opt/.style={stage, dashed},
  sub/.style={box, fill=white, font=\scriptsize, minimum height=6.5mm,
              minimum width=44mm},
  cnd/.style={box, fill=orange!12, minimum height=12mm, minimum width=28mm},
  ar/.style={->, thick, black!70, rounded corners=2pt},
  tag/.style={font=\scriptsize, inner sep=1.5pt, align=center}
]

% ---------- measurement row ----------
\node[cnd] (cand) at (1.6,0)
  {\textbf{Candidate} $c_t$\\[-2pt]%
   {\scriptsize benchmark / algorithm}};
\node[opt, minimum width=34mm] (mat) at (6.8,0)
  {\textbf{Instantiate}\\[-1pt]{\scriptsize $B = M(c_t)$}};
\node[tag] (mtag) at (6.8,1.18) {benchmark search only};
\node[sub] (ref) at (11.7,0.42) {reference run \quad $\mathcal{E}(R,B)$};
\node[sub] (alg) at (11.7,-0.42) {algorithm run \quad $\mathcal{E}(A,B)$};
\node[tag] (evl) at (11.7,1.18) {\textbf{Evaluate}};
\node[stage, minimum width=34mm] (sc) at (16.7,0)
  {\textbf{Score}\\[-1pt]{\scriptsize $g(A,B) = \mathcal{E}(R,B) - \mathcal{E}(A,B)$}};
\node[tag, anchor=north] (obj) at (16.7,-0.80)
  {$\max$ over $B$\ \ (benchmark search)\\[1pt]
   $\min$ over $A$\ \ (algorithm search)};

% ---------- panels drawn behind ----------
\begin{scope}[on background layer]
  \draw[draw=black!25, rounded corners=3pt, fill=black!4]
    (4.45,-1.72) rectangle (18.75,1.86);
  \node[box, fill=blue!8, fit=(evl)(ref)(alg), inner sep=3pt] (ev) {};
\end{scope}

% ---------- proposer: the swappable backend ----------
\node[box, fill=orange!12, minimum width=108mm] (pr) at (9.6,3.35)
  {\textbf{Propose}\ \ {\scriptsize
   $c_{t+1} \leftarrow P(c_t,\, g,\, \mathcal{R})$}\\[2pt]
   {\scriptsize \textbf{GEPA}
   \;\raisebox{-2pt}{\rule{0.4pt}{10pt}}\; \textbf{OpenEvolve}
   \;\raisebox{-2pt}{\rule{0.4pt}{10pt}}\; \textbf{coding-agent harnesses}}};

% ---------- arrows ----------
\draw[ar] (cand.east) -- (mat.west);
\draw[ar] (mat.east) -- (ev.west |- mat.east);
\draw[ar] (ev.east |- sc.west) -- (sc.west);
\draw[ar] (sc.north) |- (pr.east);
\draw[ar] (pr.west) -| (cand.north);

% an algorithm candidate skips Instantiate: it is already what gets evaluated
\draw[ar] (cand.south) -- (1.6,-1.24) -- (11.7,-1.24) -- (ev.south);
\node[tag, anchor=north] at (2.55,-1.32) {algorithm search: $A = c_t$};

\node[tag, anchor=east] at (16.4,2.32) {gap and reflections $(g,\mathcal{R})$};
\node[tag, anchor=west] at (1.78,2.32) {next candidate $c_{t+1}$};

\end{tikzpicture}}
\caption{The candidate search backend. We start with a candidate, which can be either algorithm or a benchmark(in which case we have to instantiate it), and evaluate the current benchmark set against both reference and efficient algorithm. 
Using these scores, we get a performance gap, which along with reflections generated by a reflection LLM is forwarded to a proposer backend. The proposer generates the next candidates and this loop repeats until the stopping criterion is met. 
}
\label{fig:minmaxxer-loop}
\end{figure*}

==> utility/cost_plots.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}[t]{0.48\textwidth}
\centering
\includegraphics[width=\linewidth]{images/kvpress_cursor+gepa_all_models_cost_vs_avg_best_gap.png}
\caption{FastKVZip}
\label{fig:kvpress-all-models}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.48\textwidth}
\centering
\includegraphics[width=\linewidth]{images/dca_cursor+gepa_all_models_cost_vs_avg_best_gap.png}
\caption{DCA}
\label{fig:dca-all-models}
\end{subfigure}
\caption{GEPA and Cursor agent search trajectories across models: average best gap versus cost for FastKVZip (left) and DCA (right) over 10 runs each.}
\label{fig:model-and-agent-ablation}
\end{figure*}

\galpackfalse
\renewcommand{\galpanelht}{4.00cm}
\renewcommand{\galimght}{3.55cm}
\renewcommand{\galbarht}{1.5cm}

==> utility/dca_box_1.tex <==
% Requires: tikz, tcolorbox, graphicx, booktabs, and colors defined in main.tex.
% Set \galpacktrue before \input to emit the box only (no figure*/caption).
\ifgalpack\else
\begin{figure*}[t]
\centering
\fi

\begin{tcolorbox}[
  enhanced,
  colback=boxgray,
  colframe=black!55,
  boxrule=0.55pt,
  arc=\ifgalpack 3pt\else 5pt\fi,
  width=\textwidth,
  left=\ifgalpack 2pt\else 4pt\fi,
  right=\ifgalpack 2pt\else 4pt\fi,
  top=\ifgalpack 1pt\else 3pt\fi,
  bottom=\ifgalpack 1pt\else 4pt\fi,
  title={\textbf{Context Extension via DCA}},
  fonttitle=\ifgalpack\small\else\normalsize\fi,
  coltitle=black,
  colbacktitle=black!8,
  attach boxed title to top left={xshift=8pt,yshift=-2mm},
  boxed title style={
    boxrule=0.45pt,
    colframe=black!55,
    arc=3pt,
    left=5pt,
    right=5pt,
    top=\ifgalpack 1pt\else 2pt\fi,
    bottom=\ifgalpack 1pt\else 2pt\fi
  }
]

\footnotesize

\newcommand{\dcapanel}[3]{%
\begin{tcolorbox}[
  colback=white,
  colframe=black!35,
  colbacktitle=#1,
  coltitle=black,
  title=\textbf{#2},
  fonttitle=\scriptsize,
  boxrule=0.35pt,
  arc=2pt,
  left=2pt,
  right=2pt,
  top=1pt,
  bottom=1pt,
  height=\galpanelht,
  valign=#3
]}

% ------------------------------------------------------------
% Column 1: Adversary + Validation
% ------------------------------------------------------------
\begin{minipage}[t]{0.325\textwidth}

\dcapanel{orange!15}{1. Adversary}{center}
\begin{lstlisting}[style=dcapy,numbers=none,xleftmargin=0pt,frame=none,
  basicstyle=\ttfamily\tiny,aboveskip=0pt,belowskip=0pt,
  breaklines=true,breakindent=6pt,columns=fullflexible]
def build_adversary():
    s = make_gold_str()
    put@chunk_boundary(s)
    add_distractors()
    return instance
\end{lstlisting}
\end{tcolorbox}

\vspace{\ifgalpack -2pt\else 2pt\fi}

\dcapanel{violet!12}{2. Validation}{top}
\begin{enumerate}[leftmargin=1.1em, itemsep=1pt, topsep=0pt, parsep=0pt]
  \item \textbf{By construction:} create Q/A before placing the target.
  \item \textbf{Baseline control:} keep only instances solved at native length $W$.
\end{enumerate}
\end{tcolorbox}

\end{minipage}\hspace{3pt}%

% ------------------------------------------------------------
% Column 2: Merged B0 / B1 panel
% ------------------------------------------------------------
\begin{minipage}[t]{0.325\textwidth}

\dcapanel{blue!10}{3. $B_0$ and $B_1$}{center}
\centering
\vspace{3pt}
\includegraphics[width=\linewidth,height=\galimght]{images/dcagood.png}
\end{tcolorbox}

\end{minipage}\hspace{3pt}%

% ------------------------------------------------------------
% Column 3: Evolution results + Explanation
% ------------------------------------------------------------
\begin{minipage}[t]{0.325\textwidth}

\dcapanel{green!12}{5. Evolution results}{top}
\centering
{\scriptsize
\begin{tabular}{@{}lccc@{}}
\toprule
 & $\mathcal{C}@N$ & $\mathcal{A}@\lambda N$ & Gap \\
\midrule
$B_0$ & $1.00$ & $0.90$ & $0.10$ \\
$B_1$ & $0.95$ & $0.50$ & $0.45$ \\
\bottomrule
\end{tabular}}
\end{tcolorbox}

\vspace{\ifgalpack -2pt\else 2pt\fi}

\dcapanel{yellow!18}{6. Short Explanation}{top}
\scriptsize
The evolved generator moves the target to a DCA chunk boundary and adds same-format distractors. Position remapping can fragment the target in the query's effective view, while locally coherent distractors remain competitive.
\end{tcolorbox}

\end{minipage}

\end{tcolorbox}

\ifgalpack
\vspace{-8pt}
\caption{\footnotesize
DCA adversarial-search summary. We use Llama3 (8k context length) model for 4$\times$ extension. A length-blind generator constructs matched native ($B_0$) and extended-context ($B_1$) retrieval benchmarks, validates that the native setting is solvable, and evolves examples that expose DCA's boundary sensitivity.
}
\label{fig:dca-box}%
\else
% \caption{DCA adversarial-search summary. A length-blind generator constructs matched native ($B_0$) and extended-context ($B_1$) retrieval benchmarks, validates that the native setting is solvable, and evolves examples that expose DCA's boundary sensitivity.}
% \label{fig:dca-box}
\end{figure*}
\fi
